Characterizing Improper Input Validation Vulnerabilities of Mobile Crowdsourcing Services

Mobile crowdsourcing services (MCS), enable fast and economical data acquisition at scale and find applications in a variety of domains. Prior work has shown that Foursquare and Waze (a location-based and a navigation MCS) are vulnerable to different kinds of data poisoning attacks. Such attacks can be upsetting and even dangerous especially when they are used to inject improper inputs to mislead users. However, to date, there is no comprehensive study on the extent of improper input validation (IIV) vulnerabilities and the feasibility of their exploits in MCSs across domains. In this work, we leverage the fact that MCS interface with their participants through mobile apps to design tools and new methodologies embodied in an end-to-end feedback-driven analysis framework which we use to study 10 popular and previously unexplored services in five different domains. Using our framework we send tens of thousands of API requests with automatically generated input values to characterize their IIV attack surface. Alarmingly, we found that most of them (8/10) suffer from grave IIV vulnerabilities which allow an adversary to launch data poisoning attacks at scale: 7400 spoofed API requests were successful in faking online posts for robberies, gunshots, and other dangerous incidents, faking fitness activities with supernatural speeds and distances among many others. Lastly, we discuss easy to implement and deploy mitigation strategies which can greatly reduce the IIV attack surface and argue for their use as a necessary complementary measure working toward trustworthy mobile crowdsourcing services.

==> 08_ancenstry.tex <==
Other MCS services focus on crowdsourcing family history information. For example, \textit{Ancestry.com}~\cite{ancestry} is a multi-billion company~\cite{porter_sherman_2017} which collects information about people by crawling public resources such as electorate records or marriage history databases. Its Android app has more than 5,000,000 installations and the service claims it contains more than 20 billion records and 100 million family trees. Its users can use the app to search for any individual's record. This can include one's full name, birth date, father name, mother name, and marriage information. For a non-trivial subscription fee (prices range from \$99-\$389 at the moment of writing), users can access all the above and much more for all people for whom a record exists, and more detailed records which include number and names of children, number and names of siblings, and some times residence and death information. They can also get family tree match recommendations. Below we describe a series of query injection attacks on \textit{Ancestry.com} which can lead to severe privacy leakage. All attacks are launched using \textit{spoofed networked requests}.
%Our attack on Ancestry is different from other works like \cite{edge2020attacks,ney2020genotype} on genomics apps because they show attacks on discovering some genetic data based on DNA by injecting a lot of fake data into the system whereas our attacks recover data records that are based on either data entered by the user or company's propriety data extracted from sources like school yearbooks and newspapers.

%https://www.theguardian.com/money/us-money-blog/2014/jun/19/ancestors-genealogy-high-cost-money
%A standard subscription to US data will set you back $99 a year. But if you quickly discover that your grandparents emigrated from Europe, you’re looking at $149 to $199 a year. 


% The estimated market value of Ancestry.com in 2017 was more than $3 billion

\vspace{5pt}\noindent\textbf{Manual Attack.}
We performed a man-in-the-middle (MITM) attack in a controlled environment to monitor the app's traffic when a record search request is made to the service by the user. As with the services analyzed in previous sections, this allowed us to identify the API the service exposes to its mobile applications. We found that there exists an API request (\textit{https://gateway.ancestry.com/recordservice/getrecords}) which can be used by the \textit{Ancestry.com} app for searching any record in the \textit{Ancestry.com} database. This requires knowledge of the unique-id of the record. However, we found that this id is incrementally assigned, rendering the sequence of records predictable. We also, found that there is another API (\textit{'https://gateway.ancestry.com/recordsearch/queryterm'}) that allows the client app to search records in the \textit{Ancestry.com} service by name.

Unfortunately, we were able to successfully spoof the mobile app's requests to the above APIs at the network level and mount \textit{insecure direct object reference} attacks. We found that the service accepts and responds to the spoofed requests with records including very sensitive information. This information includes PIIs such as the birth date, residence address, and gender. This is proven to be enough to uniquely identify people in the US population~\cite{sweeney2000simple}. The records also included other sensitive information such as SSN numbers and birthplace among others. SSN numbers can be used to launch identity theft attacks against individuals, while birthplace and other personal information can be leveraged for answering security questions when trying to hijack a victim's online accounts.
%\textcolor{red}{TODO: We have reported this issue to Ancestry.com and provided our recommendation for mitigating this threat.}


\vspace{5pt}\noindent\textbf{Attack Surface Characterization: Experiment Design.}
We designed two experiments, to explore the extent of privacy leakage by exploiting (a) the record id search API and (b) the name search API. 

\vspace{3pt}\noindent$\bullet$\textit{ By Record Id:} This experiment iteratively spoofs requests to the \textit{https://gateway.ancestry.com/recordservice/getrecords} API. Each request uses a record id starting from 1 up to 10,000.

\vspace{3pt}\noindent$\bullet$\textit{ By First Name:} This experiment iteratively spoofs requests to the \textit{https://gateway.ancestry.com/recordsearch/queryterm} API, using a new name each time as the query term. Since we do not know what names are in the \textit{Ancestry.com} database, we used a name dataset~\cite{railsmec91:online}. This dataset contains 89372 First names in total. We randomly sampled this dataset and spoofed queries for 57,000 names. We regard a query successful when it is accepted by the service and the service responds to it with records. For each successful query, we collect the top 100 records returned. We retrieve a maximum of 100 records per name by specifying it as a parameter of the query we are employing and we make sure the records returned are specific to the name we searched by specifying another parameter of the query which determines the strictness of the matching while searching the records corresponding to the first name.

%The second experiment involved searching an API call that can be used to search a first name in the database of records. We took a dictionary of names from different countries and searched 57,000 names with a parameter of 100 results per name to the API call.

%One of the problems that we encountered while trying to spoof the network request detailed above, was that the requests were using an authentication token which expired after every one hour.  Because of this, some of our experiments needed to be run for about 31 hours. However, after further investigation, we found another API request that employed a client-secret for acquiring a new authentication token for the app. We exploited this to keep getting new authentication tokens and keep spoofing requests without getting blocked. 

\vspace{5pt}\noindent\textbf{Attack Surface Characterization: Results.}
In launching the attacks we observed that the victim service interface had a serious flaw which allows an adversary to expose highly sensitive information that is supposed to be revealed only to premium accounts. In particular, the service responded to our spoofed queries with all the information the service has about a record. This information is filtered by the mobile app according to the account type the user has (free vs premium). This might be a system performance decision as computation is delegated to the client nodes. However, we showed that in tandem with our request spoofing attack, this can be exploited by an adversary to effectively mirror \textit{Ancestry.com}'s database. Adversaries or opportunistic users can also exploit this to get access to paid services for free severely affecting \textit{Ancestry.com}'s revenue streams. 

Table~\ref{tab:ancenstry_byrecordid_all} shows the fields and their frequency we were able to uncover by spoofing 10,000 request queries \textit{by record id}. First, we observe that each of our requests reveals a new unique record (for a total of 10,000 records). We also, see that big proportions of field types are supposed to be available only to premium numbers but we managed to expose that information: 9611/10000 (96\%) of SSN numbers, 9610/9999 (96\%) of birth dates, 342/351 (97\%) of gender, 3896/5327 (73\%) of birthplaces among others, are supposed to be hidden from free accounts but are leaked. 
%We also managed to extract the types of information records the service utilized for collecting the information revealed with the attack by record id which we list on  Table~\ref{tab:ancenstry_byname_recordtypes} in the Appendix~\ref{app:familyHistory}.

\begin{table}[ht]
\vspace{-7pt}
\centering
\scriptsize
\caption{Ancestry: Information Leakage by Record ID}
\label{tab:ancenstry_byrecordid_all}
\begin{tabular}{ l | l | l }
\toprule
 \textbf{Fields} & \textbf{Leaked Freq.}          &  \textbf{Total Freq.} \\ \hline
Full Name & - & 9998 \\
Gender & 342 & 351 \\ 
Notes & 9611 & 10000 \\ 
Father & 89 & 94 \\ 
Birth Place & 3896 & 5327 \\ 
SSN & 9611 & 10000 \\ 
Mother & 88 & 94 \\ 
Death Date & 2916 & 3044 \\ 
Claim Date & 9339 & 9716 \\
Birth Date & 9610 & 9999 \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}

Table~\ref{tab:ancenstry_byname_selected} lists some of the fields leaked to the our attack by spoofing 57,000 \textit{names}. We observe that our approach is highly effective and we were able to reveal records that included sensitive information such as full names, birth dates, and relationships with other people (spouses, siblings, and parents). As before, we further observe that with this method, also big proportions of field types which are supposed to be available only to premium numbers are leaked: $3022626/3168821$ ($95.4\%$) of marriage certificates, 879587/922177 (95.4\%) of birth dates, 54951/57608 (95.4\%) of mother names, 164852/172820 (95.4\%) of father names, 54956/57611 (95.4\%) of spouses' birth year among others. A full list of fields revealed with the attack by name is provided on Table~\ref{tab:ancenstry_byname_all} in the Appendix~\ref{app:familyHistory}.


\begin{table}[]
\centering
\scriptsize
\caption{Ancestry: Information Leakage by First Name}
\label{tab:ancenstry_byname_selected}
\begin{tabular}{ l | l | l}
\toprule
 \textbf{Fields} & \textbf{Leaked Freq.}          &  \textbf{Total Freq.} \\ \hline
Full Name & - & 5761498 \\ 
Birth & 879587 & 922177 \\
Residence & 377 & 453 \\ 
%Vital \textcolor{red}{??} & 164879 & 172846 \\ \hline
Marriage & 3022626 & 3168821 \\ 
Spouse & - & 1613376 \\ 
Spouse Birth Year & 54956 & 57611 \\ 
Spouse Residence Place & 20 & 20 \\ 
%Spouse Residence \textcolor{red}{??} & 3 & 3 \\ \hline
%Parent & 2 & 3 \\ \hline
%Bond date & 7 & 7 \\ \hline
%Widow's Death Place & - & 1 \\ \hline
%Departure & 1 & 7 \\ \hline
%Spouse Birth Place & 1 & 57611 \\ \hline
Father & 164852 & 172820 \\ 
Mother & 54951 & 57608 \\ 
%Military & - & 1 \\ \hline
%Origin & 1 & 3 \\ \hline
%Date Discharged & - & 1 \\ \hline
%Civil & - & 4 \\ \hline
%Widow's Death Date & - & 1 \\ \hline
Children & 21 & 23 \\ 
Relative & 6 & 36 \\ 
%Arrival \textcolor{red}{??} & 12 & 35 \\ \hline
Death & 140 & 166 \\ 
%Sibling & 4 & 4 \\ \hline
%Bond Place & - & 7 \\ \hline
%Spouse Birth Location & - & 2 \\ \hline
\bottomrule
\end{tabular}
\vspace{-7pt}
\end{table}

\iffalse
\begin{table}[]
\centering
\caption{Ancestry: Attack2 Veiled Fields}
\label{tab:inputTypes5}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Arrival & 12 \\ \hline
Origin & 1 \\ \hline
Death & 140 \\ \hline
Bond date & 7 \\ \hline
Parent & 2 \\ \hline
Sibling & 4 \\ \hline
Residence & 377 \\ \hline
Father & 164852 \\ \hline
Departure & 1 \\ \hline
Spouse Residence Place & 20 \\ \hline
Relative & 6 \\ \hline
Spouse Residence & 3 \\ \hline
Vital & 164879 \\ \hline
Marriage & 3022626 \\ \hline
Spouse Birth Place & 1 \\ \hline
Birth & 879587 \\ \hline
Mother & 54951 \\ \hline
Spouse Birth Year & 54956 \\ \hline
Children & 21 \\ \hline
\end{tabular}
\end{table}
\fi



==> 12_app_ancenstry.tex <==
\label{app:familyHistory}


\iffalse
\begin{table}[]
\centering
\caption{Ancestry: Attack1 Record Categories}
\label{tab:ancenstry_byrecordid_recordtypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Court, Governmental, Criminal Records & 10000 \\ \hline
\end{tabular}
\end{table}
\fi

Table~\ref{tab:ancenstry_byname_all} provides the full list of fields, along with their frequencies, that were searched and uncovered with our attack by first name on \textit{Ancestry.com} (Section~\ref{sec:ancenstry}).

\begin{table}[]
\centering
\footnotesize
\caption{Ancestry: Information Leakage by First Name}
\label{tab:ancenstry_byname_all}
\begin{tabular}{ l | l | l }\toprule
 Fields & Leaked Freq.          &  Total Freq. \\ \hline
Death & 140 & 166 \\
Father & 164852 & 172820 \\ 
Spouse Residence & 3 & 3 \\ 
Vital & 164879 & 172846 \\ 
Arrival & 12 & 35 \\ 
Parent & 2 & 3 \\ 
Birth & 879587 & 922177 \\ 
Spouse & - & 1613376 \\ 
Spouse Birth Year & 54956 & 57611 \\
Bond date & 7 & 7 \\ 
Name & - & 5761498 \\ 
Widow's Death Place & - & 1 \\ 
Residence & 377 & 453 \\ 
Departure & 1 & 7 \\ 
Spouse Residence Place & 20 & 20 \\
Marriage & 3022626 & 3168821 \\ 
Spouse Birth Place & 1 & 57611 \\ 
Mother & 54951 & 57608 \\ 
Military & - & 1 \\ 
Origin & 1 & 3 \\ 
Date Discharged & - & 1 \\
Civil & - & 4 \\
Widow's Death Date & - & 1 \\
Relative & 6 & 36 \\ 
Sibling & 4 & 4 \\ 
Bond Place & - & 7 \\ 
Spouse Birth Location & - & 2 \\ 
Children & 21 & 23 \\ 
\bottomrule
\end{tabular}
\end{table}


\iffalse
\begin{table}[]
\centering
\footnotesize
\caption{Record Categories Ancestry Used to Collect the Leaked By Name fields.}
\label{tab:ancenstry_byname_recordtypes}
\begin{tabular}{ l | l }\toprule
 Fields          &  Times Found \\ \hline
1900s (Decade) & 24 \\ 
Birth, Baptism \& Christening & 115356 \\ 
Draft, Enlistment and Service & 41 \\ 
1830s & 4 \\ 
Passenger Lists & 10 \\ 
1880s & 3 \\ 
1940s & 14 \\ 
1920s & 141 \\ 
Soldier, Veteran \& Prisoner Rolls \& Lists & 7 \\ 
Citizenship Records & 21 \\
1850s & 2 \\
1930s & 70 \\ 
1870s & 9 \\ 
1860s & 6 \\ 
Death, Burial, Cemetery \& Obituaries & 241 \\
Marriage \& Divorce & 5645501 \\
Pension Records & 2 \\ 
Court, Governmental \& Criminal Records & 10 \\
1910s & 34 \\
1840s & 3 \\
\bottomrule
\end{tabular}
\end{table}
\fi

==> 12_app_extra_tables.tex <==
%%%%%%%%%%%%% API table starts %%%%%%%%%%%%%%%
\vspace{5pt}\noindent\textbf{Successful Injections.} Table~\ref{tab:num_injections} lists the number of successful injections per service and targeted interface performed throughout our experiments.

\begin{table}[htbp!]
\centering
\footnotesize
\caption{Number of successful input injections.}
\label{tab:num_injections}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\textbf{Service}              & \textbf{No. Installations} & \textbf{Domain} & \textbf{Input Injections} & \textbf{Interface} \\ \hline
Strava                        & 10,000,000+ & Fitness Service & 708     & Web API       \\
Fitbit                        & 50,000,000+ & Fitness Service & 98      & Web API       \\
Map My Run                    & 10,000,000+ & Fitness Service & 797     & Web API       \\
Basket Savings                & 100,000+ & Pricing Service & 156     & Web API       \\
ToiFi (Toilet Finder)         & 50,000+ & Location-Based Service & 2728    & Web API       \\
Police Detector               & 5,000,000+ & Location-Based Service & 2668    & Web API       \\
Transit                       & 5,000,000+ & Transportation Service & 403     & Sensor        \\
Neighbors By Ring             & 1,000,000+ & Safety Service &  113    & App UI        \\
Google Maps                   & 5,000,000,000+ & Transportation Service &    1000     &     App UI, Sensor     \\
Gas Buddy                     & 10,000,000+ & Pricing Service &   ~800  & Sensor        \\
\end{tabular}%
}
\end{table}
%Ancestry & 67000 & Web API\\

\ignore{
%\multicolfloat{
%\begin{landscape}
\begin{table*}[tp!]
\centering
\caption{Web APIs discovered for different mobile crowdsourcing services.}
\label{tab:api_calls}
%\resizebox{\columnwidth}{!}{%
\resizebox{\linewidth}{!}{%
%\resizebox{\textwidth}{!}{%
%\resizebox{17cm}{!}{%

\begin{tabular}{l|l|l}
\toprule
\textbf{APP}                      & \textbf{API Function}              & \textbf{API Call}                                                                         \\ \hline
\multirow{4}{*}{Strava}           & Add activity.                      & https://m.strava.com/api/v3/activities                                                    \\ \cline{2-3} 
                                  & Get user stats.                    & https://m.strava.com/api/v3/athletes/user-id/stats                                        \\ \cline{2-3} 
                                  & Get user profile.                  & https://m.strava.com/api/v3/athletes/user-id/profile?hl=en\_US                            \\ \cline{2-3} 
                                  & Get user goals.                    & https://m.strava.com/api/v3/athletes/user-id/progress-goals?                              \\ \hline
\multirow{4}{*}{Fitbit}           & Add Run(or other activity).        & https://android-cdn-client.fitbit.com/1.1/user/-/activities.json                          \\ \cline{2-3} 
                                  & Get activities for day.            & https://android-cdn-api.fitbit.com/1.2/user/-/activities/date/date.json                   \\ \cline{2-3} 
                                  & Search activity types.             & https://android-cdn-api.fitbit.com/1.1/user/-/activity/search.json?q=                     \\ \cline{2-3} 
                                  & Get user goals.                    & https://android-cdn-api.fitbit.com/1/user/-/exercises/goals/summary.json?                 \\ \bottomrule
\multirow{6}{*}{Map My Run}       & Add new run.                       & https://uarun-mobile.api.ua.com/v7.2/workout/                                             \\ \cline{2-3} 
                                  & Get weekly user stats.             & https://uarun-mobile.api.ua.com/v7.2/user\_stats/user-id/                                 \\ \cline{2-3} 
                                  & Find workout details.              & https://uarun-mobile.api.ua.com/v7.2/workout/workout-id/                                  \\ \cline{2-3} 
                                  & Get User profile details.          & https://uarun-mobile.api.ua.com/v7.2/user/user-id/                                        \\ \cline{2-3} 
                                  & Get challenges joined.             & https://uarun-mobile.api.ua.com/v7.2/challenge/?joined=true\&-user=                 \\ \cline{2-3} 
                                  & Get user gear.                     & https://uarun-mobile.api.ua.com/v7.2/usergear/?user\_id=user-id                           \\ \hline
\multirow{7}{*}{Basket Savings}           & Add price.                         & https://api.basketsavings.com/pricesnap/app/product/price/add                             \\ \cline{2-3} 
                                  & Get product prices in radius.      & https://api.basketsavings.com/basket-api/product/analysis?productId=product-id            \\ \cline{2-3} 
                                  & Get product boundaries for store.  & https://api.basketsavings.com/basket-api/oob?productId=product-id\&storeId=store-id       \\ \cline{2-3} 
                                  & Get store details.                 & https://api.basketsavings.com/basket-api/store/details/store-id                           \\ \cline{2-3} 
                                  & Search products.                   & https://api.basketsavings.com/basket-api/search/product/price/minimal?keyword=eggs        \\ \cline{2-3} 
                                  & Similar products from other brand. & https://api.basketsavings.com/basket-api/product/analysis/similar/other\_brand?productId= \\ \cline{2-3} 
                                  & Similar products from same brand.  & https://api.basketsavings.com/basket-api/product/analysis/similar/same\_brand?productId=  \\ \hline
\multirow{5}{*}{ToiFi (Toilet Finder)} & Add toilet.                        & https://api.toiletfinder.xyz/toilets                                                      \\ \cline{2-3} 
                                  & Get toilets.                       & https://api.toiletfinder.xyz/toilets                                                      \\ \cline{2-3} 
                                  & Report toilet doesn't exist.       & https://api.toiletfinder.xyz/toilets/toilet-id/nonExistent                                \\ \cline{2-3} 
                                  & Report toilet isn't clean.         & https://api.toiletfinder.xyz/toilets/toilet-id/requestCleaning                            \\ \cline{2-3} 
                                  & Toilet details and reviews.        & https://api.toiletfinder.xyz/toilets/toilet-id/reviews?limit=10\&offset=0                 \\ \hline
\multirow{4}{*}{Police Detector}  & Register device.                   & http://194.58.102.65/reg.php                                                              \\ \cline{2-3} 
                                  & Add POI.                           & http://142.11.196.19/input.php                                                            \\ \cline{2-3} 
                                  & Get POIs.                          & http://142.11.196.19/output.php                                                           \\ \cline{2-3} 
                                  & Delete POIs.                       & http://142.11.196.19/input.php (with pos\_type=0 in request body)                         \\ \hline
%\multirow{3}{*}{Ancestry}         & Search records by ID.              & https://gateway.ancestry.com/recordservice/getrecords                                     \\ \cline{2-3} 
%                                  & Search records by first name.      & https://gateway.ancestry.com/recordsearch/queryterm                                       \\ \cline{2-3} 
%                                  & Get new access token.              & https://auth.ancestry.com/oauth20/tokens                                                  \\ \hline
\end{tabular}
}
\end{table*}
%\end{landscape}
%}
%%%%%%%%%%%%% API table ends %%%%%%%%%%%%%%%
}

==> 12_app_gas.tex <==
Similar to basket, gasBuddy is a crowdsourcing platform for comparing prices of gas at different
gas stations. They get their data from their users who report price changes for gas at any
particular gas station.
The attack is to increase or decrease cars to a particular gas station by increasing or decreasing
prices of gas significantly.
Alternatively, we can find out how much the gas prices can be altered by fuzzing the inputs.

\vspace{5pt}\noindent\textbf{Experiment Design.}
This experiment was conducted using an appium script. One phone was used for both injecting and observing the price change. We took four gas stations which were Mobil, ACRO, 76 and Chevron gas stations and found the maximum and minimum price range for the regular gas on these stores. We initially tried the exponential increase or decrease strategy followed by iterative increase or decrease but noticed that the same amount of increase or decrease isn't allowed in all iterations so we went with an increase or decrease of 1 cent in each iteration consequently.

\vspace{5pt}\noindent\textbf{Attack Characterization.}
The results are shown in the corresponding table 5.

\begin{table}[h]
\centering
\caption{GasBuddy Regular Gas Results}
\begin{tabular}{llll}
Product                           & Value & Max & Min \\
Mobil             & 2.93 & 3.33 & 2.75 \\
ARCO            & 2.73 & 3.19 & 2.59 \\
76       & 2.95  & 2.95 & 2.94 \\
Chevron               & 3.15 & 3.15 & 3.15 
\end{tabular}
\end{table}

==> 12_app_injections_table.tex <==
\begin{table}[]
\centering
\caption{Number of Injections per app using API calls.}
\label{tab:num_injections_old}
\begin{tabular}{l|l} \toprule
\textbf{App}              & \textbf{Number of Injections by API} \\\hline
Police Detector  & 2668                        \\
Toifi Toilet App & 2728                        \\
Strava           & 708                         \\
Fitbit           & 98                          \\
Map My Run       & 797                         \\
Basket           & 156                          \\\bottomrule                     
\end{tabular}
\end{table}




==> 12_app_nbr.tex <==
%Examples of generated posts accepted by the \textit{Neighbors by Ring}
%\label{app:nbr_examples}
%\vspace{0pt}\noindent\textbf{Neighbors by Ring: Successful Injections Examples.} 
Table~\ref{tab:accfakex} lists some representative examples of fake posts we generated with the SGP and SGA models, and accepted by \textit{NbR}. Table~\ref{tab:num_injections} lists the number of successful injections per service and targeted interface performed throughout our experiments.


%Ancestry & 67000 & Web API\\


==> 12_app_similar_apps.tex <==
\section{Similar Apps}
\label{app:similar_apps}

The apps in this table are also similar to the apps that we studied in depth in our experiments. We collected them by either 1)Searching up the apps that we studied on google play store and then recursively looking up apps related to them and then apps related to the related apps and so forth. 2) Searching the category of the apps we studied on google play store, choosing some apps and then recursively finding more apps like the previous way.

\begin{table}[]
\begin{tabular}{ll}
\textbf{Type}                                              & \textbf{Apps}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{|l|}{Neighborhood.}                        & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}OLIO - Share more. Waste less,\\ Nextdoor: Local News, Garage Sales \& Home Services,\\ Ring - Always Home,\\ Naber - Neighborhood Watch,\\ SaferWatch,\\ Neighbor,\\ Nextdoor for Public Agencies,\\ Neighborhood Crime Watch,\\ Hoplr - Get in touch with your neighbours,\\ WeAlert – safer neighborhoods,\\ PulsePoint AED,\\ SpotCrime+ Crime Map\end{tabular}}                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{Transportation.} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}MyTransit NYC Subway, Bus, Rail (MTA),\\ Citymapper,\\ Google Maps,\\ Waze,\\ City Transit: Live Public Transport, Routes, Fare,\\ MTA Bus Time,\\ NYC Live Bus Tracker \& Map\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{Family History}                       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Find A Grave,\\ Heredis,\\ GEDexplorer,\\ Genoom,\\ Kinsmap,\\ Quick Family Tree,\\ FamilySearch Tree,\\ FamilySearch Memories\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{Fitness}                   & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}adidas Running app by Runtastic,\\ Endomondo - Running \& Walking,\\ Running App - Run Tracker with GPS, Map My Running,\\ Running \& Jogging,\\ Sportractive GPS Running Cycling Distance Tracker,\\ Runkeeper - GPS Track Run Walk,\\ Running Distance Tracker +\end{tabular}}                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{Nearby Utility}                       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Where is Public Toilet,\\ Free WiFi Passwords \& Hotspots by Instabridge,\\ Free WiFi Passwords \& Internet Hotspot by WiFi Map,\\ Earthquake Network - Realtime alerts,\\ Radar \& Detector police, camera, work,traffic 2020,\\ Police Radar (Speed Camera Detector),\\ Police Speed \& Traffic Camera Radar \& Detector,\\ Police Detector, Radar, Blitz Camera \& Alert,\\ Speed Cameras Radar,\\ Radarbot Free: Speed Camera Detector \& Speedometer,\\ Speed Camera Detector Free,\\ Toilet Finder,\\ Public Toilet Finder | No. 1 Restroom Locator,\\ Flush - Find Public Toilets/Restrooms,\\ SitOrSquat: Restroom Finder\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{Money Saving}                         & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Gas Buddy,\\ GetUpside: Earn Money \& Get Gas Prices Near You,\\ Gas Guru: Cheap gas prices,\\ Checkout 51: Gas Rewards \& Grocery Cash Back,\\ Receipt Pal: Shop, Earn Paid Rewards \& Gift Cards,\\ Fetch Rewards: Shop, Snap, Win,\\ Receipt Hog - Receipts to Cash\end{tabular}}                                                                                                                                                                                                                                                                                                                                                            \\ \hline
      
\end{tabular}
\end{table}
    

==> 12_app_toifi.tex <==
%\subsection{Attacks on ToiFi (Toilet Finder)}
%\label{app:toifi}
\vspace{5pt}\noindent\textbf{ToiFi (Toilet Finder)}~\cite{PublicTo19:online} is a location-based MCS which allows users to find public restrooms (as PoIs) in time of need. It allows participants to add new or edit/remove previous PoIs. Its Android app was installed more than 50,000 times. We were successful in both manually adding and removing PoIs at arbitrary locations. To systematically characterize the attack surface of the service next we use the \textit{GPS coordinates exploration} strategy to discover the range of coordinates that can be used to fake a public toilet. To conduct the experiments we identified---through our MITM proxy---the API the remote service exposes for receiving a request to add a PoI. We then carefully craft network requests triggering the API, by spoofing the mobile app and a service user. Success of the injection is determined by spoofing a second request targeting a different exposed API which allowed us to search for the presence of a PoI. We found that out of bound longitudes and latitude values (CE-O) are rejected. However, all trials on \textit{CE-Long}, \textit{CE-Lat} and \textit{CE-2D} were successful allowing us to inject PoIs anywhere on the surface of the Earth. For \textit{CE-Prec}, we saw that we can inject POIs up to a precision of 7 decimal places for both longitude and latitude. Furthermore, we noticed that there is no check preventing two points from being too close on the map as the first round of injections went fine as it is. Evidently, this can be exploited for fun, for example by injecting toilets in the middle of the desert or in the middle of the ocean. It can also be used for pranks as public toilets can be injected on a target individual's or enterprise's private premises; or even for harm, as people can be lured in dark alleys and isolated areas. We marked all PoIs added by our experiments as non existent by spoofing another API call we discovered so as to not harm the service or its users.

%\textit{https://api.toiletfinder.xyz/toilets/toilet-id/nonExistent} so as to not harm the service or its users.
%(https://api.toiletfinder.xyz/toilets). We then carefully craft network requests triggering the API, by spoofing the mobile app and a service user. Success of the injection is determined by spoofing a second request (https://api.toiletfinder.xyz/toilets) targeting a different exposed API which allowed us to search for the presence of a PoI. We found that out of bound longitudes and latitude values (CE-O) are rejected. However, all trials on \textit{CE-Long}, \textit{CE-Lat} and \textit{CE-2D} were successful allowing us to inject PoIs anywhere on the surface of the Earth. For \textit{CE-Prec}, we saw that we can inject POIs up to a precision of 7 decimal places for both longitude and latitude. Furthermore, we noticed that there's no check preventing two points from being too close on the map as the first round of injections went fine as it is. Evidently this can be exploited for fun, for example by injecting toilets in the middle of the desert or in the middle of the ocean. It can also be used for pranks as public toilets can be injected on a target individual's or enterprise's private premises; or even for harm, as people can be lured in dark alleys and isolated areas. We marked all PoIs added by our experiments as non existent by using the API call \textit{https://api.toiletfinder.xyz/toilets/toilet-id/nonExistent} so as to not harm the service or its users.

==> 13_gas_buddy.tex <==
GasBuddy is another tech company that provides its users with real-time fuel prices through their Android app. It operates in the United States, Canada, and Australia and has more than 140,000 gas stations covered in its database. We found out that it uses crowd-sourcing and relies on user reports to find out the real-time fuel prices for different gas stations. Like google maps, it also had the client pinning defense in place so we couldn't get decrypt and reverse engineer the api calls used by the app. This hindered us from scaling up the experiments. However, we did some automated experiments on four different gas stations and found out that the prices of gas can be increased or decreased by one to two dollars if changed one cent at a time(per injection) whereas a drastic change in price in one injection gets rejected. We also couldn't scale this experiment more because of the variable nature of gasBuddy's user interface where random pops would cause the app to crash or end up at unintended screens frequently.

==> 14_google_maps.tex <==



Google Maps is an online mapping service provided by Google. It offers its users a number of features like route planning, satellite imagery, aerial photography and to our most interest real-time traffic conditions. We believe that these traffic condition estimations are based on crowd sourced data. We tried to perform experiments with Google Maps to see if we could perform similar data poisoning attack but couldn't succeed for a few reasons. First, we couldn't reverse engineer the api calls used by the google maps android app since the app uses client certificates to avoid decryption of its api calls. This made conducting the experiments at scale harder. Secondly, we tried walking around our university campus with both fake emulators and 10 real phones in the middle of the night to see if we could alter the view of a third observer for how busy the roads are but the view didn't change. We think this is because 10 phones weren't enough to cross the threshold for getting road classified as busy by the google servers. This popular news article \cite{barrett} from a few months ago however shows how a person carrying 99 phones in a wagon could simulate a fake traffic jam on google maps.

==> old_defence.tex <==
Based on our observations we propose that simple strategies for \textit{input domain restrictions} and \textit{semantic validation} can greatly reduce the attack surface and the actual repercussions of poisoning attempts. 

For example, this did x for the x app; this check reduced the number of poisoned values from x to x ofr this app. etc.

These restrict the adversary into injecting realistic values which greatly limit the damage to training data poising attacks for machine learning models. However, detecting fake values that look realistic is a hard problem as we also show in \textit{Neighbors by Ring}, where a more sophisticate adversary can bypass even semnatic verification. We need further solutions with stronger client authentication, and user verification.  Solutions from trusted computing (accountability and defense against network adversaries) can limit scalability of attacks but still a malicious user could manually poison inputs. CONS: Universality - not all phones have trusted hardware; and Backward compatibility: OS needs to expose APIs for using trusted hardware.
User ratings and reputation schemes can also help. These suffer from slow start. Also in some cases we would want to take into account new data from new users (examples?).


%%Neighbor 
\subsection{Neighbor by Ring}
The app \textit{Neighbor by Ring} has put in place some level of semantic validation against potential fraudulent or irrelevant entries. However, with today's state-of-the-art text generation tools we have shown in Section \ref{sec:safety} that it is possible to inject fake posts for all category types. Moreover, the minimal form of verification (email only) is easy to by pass by creating new temporary accounts when blocked. Additionally, the attacker does not need to have a physical and valid address.   
Nevertheless, several mechanisms can be put in place to fortify the app's security. First of all, adding a compulsory verification via phone number would make it already harder to create new accounts. Another but more costly option \textcolor{purple}{[ Need to check how pricy]}, is to send via post mail secret keys to validate the physical address. The app could also function with a 'upvote' system that neighbours could confirm the validity for claims such as fires or shootings.  Neighbour could also be selected based on their GPS location and be asked about the situation in their surroundings. Of course, if an attacker can create multiple accounts and spoof their GPS sensor, they could interfere here as well. 
Finally, although models like GPT2 can generate text with a distribution that  resemble humans', it can still be detected with models such as GPT-2 Output Detector \cite{solaiman2019release}. This model a distilled model of BERT, RoBERTa, trained on a dataset of GPT2 output to identify non human text. We tested this model on our crawled posts and 486 out of 1080 (45\%) were falsely detected as fake. We then gave our accepted fake posts as an input to the model and 55 were classified as false out of 97 (57\%).


\vspace{5pt}\noindent\textbf{Domain and Semantic Restrictions.}
\subsection{Fitness Apps}
We can restrict the input domain for these apps by two ways. The first restriction is on the total distance allowed for one run and is set to be 350 miles which is the world record for the longest non-stop run by Dean Karnazes. The second restriction is on the average speed of the run which can't exceed 27.9617 miles per hour (45 kilometer per hour) which is still slightly above Usain Bolt's world record of 27 miles per hour. This can be further restricted by semantic validation too. Furthermore for input domain restriction for the swimming and cycling activities on Strava specifically, the maximum distances allowed would be 139.8 miles (Veljko Rogošić's world record) and 3,020 miles (Christoph Strasser's world record)  respectively while the total average speeds allowed will be 5.122584 miles per hour (Tom Jager's world record) and 183.9 miles per hour (Denise Mueller-Korenek's world record) respectively.   These apps can use the data collected by its user for their run's and leverage it to detect fraudulent injections as anomalies. It can see if each injected run lies within 3 standard deviations of the average running distance and duration for the user's gender and age.
\subsubsection{Map My Run}
We see that the input domain gets reduced to $0.35$ percent of its original value by the first domain restriction strategy alone for running. (Original max distance is 100051.4 miles)

\subsubsection{Fitbit}
We see that the input domain gets reduced to $3.5$ percent of its original value by the first domain restriction strategy alone for running. (Original max distance is 10,000 miles)

\subsubsection{Strava}
We see that the input domain gets reduced to $0.0011$ percent, $0.0004$ percent, $0.0.0096$ percent, of its original value, for running, swimming and cycling respectively, by the first domain restriction strategy alone for running. (Original max distance is 31622400 for all activities)

\subsection{Location Based Apps}
For these apps, we can do the input domain restriction validation in two steps. The first step is to not allow any values that lie beyond the boundaries for longitudes (-180.0 to 180.0) and latitudes (-90.0 to 90.0). The second step is to validate that these longitudes and latitudes do not correspond to points that lie in any of the oceans or Antarctica. We can further limit the injection possibilities by semantic validation for the two apps as follows:

\subsubsection{Toifi Toilet App}
The semantic validation for this app can be done by using OpenStreetMap's data to validate if the injected values of longitudes and latitudes do in fact lie within a city or otherwise within a certain distance of highways and roads. If, they are not we can reject these values for toilets.

\subsubsection{Police Detector}
Similar to the Toifi Toilet App, the semantic validation for this app leverages OpenStreetMap's data to validate if the injected values of longitudes and latitudes lie on a street or a road. If they don't, we can reject the injected point.

\subsection{Ancestry}
This app can get significantly more secure by employing the following three defenses. First, restrict the number of queries that a user can make per day. Second, block the user that is trying to make more than the upper limit of queries allowed per day or is making a lot of queries in a very short time i.e detect and block crawling. Third, process what data is the non-paid member allowed to see on server side instead of the client side. This, third defense would safeguard their app against people using their paid service for free.\\
Lets consider the first defense, employing it and imposing a limit to be able to search 20 names only per day would reduce the attack surface to $0.00035$ percent of how much we showed that can be crawled. (Original max searchhes we did were for 57000 first names).

\subsection{Transit}
Charles can handle this better. For GPS spoofing detection, can take inspiration from uber's defense article here https://eng.uber.com/advanced-technologies-detecting-preventing-fraud-uber/ and for fingerprinting fraudulent or bot-behavior because of our appium script, can take help from lyft's article here https://eng.lyft.com/fingerprinting-fraudulent-behavior-6663d0264fad.

\subsection{Basket}
For input domain restriction on this app, we can use 70 percent of a products current value as the minimum possible value and 130 percent of a product's current value as the maximum possible value. This is a much tighter bound than the bound observed, for most products, which is $10$ percent of the product's current value for the minimum possible allowed value and $2 * ceil(current-value)$ for the maximum possible value. We assume that its unreasonable for any product to fluctuate more than 30 percent of its current value under normal circumstances. Furthermore, semantic validation can be done by seeing how far does the injected value lie from the mean of all previously injected values for that product. The first defense alone would significantly reduce the attack space. For instance, for a gallon of milk which is priced at 3.49 dollars and has the minimum and maximum possible values of 0.35 and 8.0 dollars respectively, the input domain restriction defense would reduce the injection space by $72.63$ percent.

==> old_framework/3_framework.tex <==
%FRAMEWORK DESIGN
To help us systematically characterize the attack surface of mobile croudsourcing apps, we design an analysis framework. Our framework, named \systemName{}, assumes a threat stems from a malicious participating mobile device or its user. Next we elaborate on the threat model we consider, the design challenges of such a framework and lastly on how we overcome those challenges in \systemName{}.

\subsection{Threat Model.} We consider an adversary with access to the mobile app of the target ubiquitous crowdsourcing service. We also assume the adversary can observe the traffic generated between the app and the remote service either by passive eavesdropping or active man in the middle attacks. She can also reverse engineer and analyze the mobile app interfacing with the service. Thus the adversary is in knowledge of the communication protocol and can leverage it to try to inject fake data into the service. However, the adversary has no access to the remote service and can only treat it as a black box. 
%This is both a realistic and a strong adversary as it only assumes access to freely available information and tools; and requires low effort.

\subsection{Design Challenges.} To characterize the attack surface or popular services, we need a systematic way to identify what such an adversary can inject and under what conditions. One could merely subscribe to the service and use its mobile app to manually perform the data injection. This approach does not scale very well since it would be very cumbersome to try all possible input values under all possible conditions for every service. Consider for example \textit{Basket Savings}. The analyst would need to first navigate to the screen that corresponds to the store of interest. Then she will need to look for the item of interest and click on it. After that she will finally be able to input a new price for the item and submit it. To make things worse, this process needs to be repeated for all possible float values $x$ of price ($x \in \R$), and for all items of interest ($i \in I_s$, where $I_s$ is the set of all items in store $s$, ($s \in S$)). This would require $|\R| \times |I| \times |S|$ manual experiments. Consider these in the context of the recent case of Google Maps~\cite{cartPhonesGM} where we also require 100 real phones. Evidently we need an automated and systematic way of performing such experiments.

This is not a trivial endeavor. In fact we encountered three main challenges in scaling up the characterization process: (1) Poisoning the data; (2) the black-box nature of crowdsourcing services; and for some cases (3) navigating to the application's screen of interest. 

\vspace{5pt}\noindent\textbf{Data Poisoning.} We need a reliable way to inject input values to the target service. This requires good knowledge of the communication protocol between the service and the participating nodes. In almost all cases this communication is encrypted which hinders the monitoring process. Moreover, spoofing networking requests is not always easy. For example, a number of apps use \textcolor{red}{certificate pinning} at the server which renders any MITM approaches ineffective. In such cases we leverage the fact that the official app can communicate with the service and attempt the injection through the application. Assuming we solve the \textit{navigation} challenges and land on the mobile app's screen where the injection can happen, we face user interface analysis challenges as we need a reliable way to identify the UI element the automated tool should interact with (in this case to input a value of a particular input type). To make things worse, not all apps/services collect input through the UI. Some collect real-time measurements from IMU and localization sensors or \textcolor{red}{follow a hybrid approach where UI inputs are coupled with sensory input like in the case of Neighborhood Safety.}. If our tool is restricted to the UI we would be missing on reporting on a number of possible injection opportunities. Thus we need to be able to generate and send sensory input measurements, inject inputs to UI elements and in some cases coordinate the two to happen synchronously. 

\vspace{5pt}\noindent\textbf{Black Box Crowdsourcing Services.} Succeeding in posting a value to the service does not necessarily mean that this value is accepted and used by the service. However, we cannot have access to the internal algorithms of the services, and we can only use them as a black box. Thus, we focus on monitoring a service's reaction to systematically generated triggering requests. We found that a lot of services are using some verification measures to mitigate spoofing attempts, which renders response monitoring challenging. For example, some services (e.g. \textcolor{red}{Basket Savings}) are blocking requests from emulator devices while others (e.g. \textcolor{red}{Neighborhood Safety}) use more sophisticated approaches to detect suspicious posts. Even after we tackle these data verification challenges, we still need a way to determine whether the injected measurement was not only accepted but actually had an effect on the service. Again, this cannot always happen through the network and thus we further need a reliable strategy to monitor the UI interface. To make things worse, in some cases, the UI of the device where the injection takes place might be updated to reflect the injected information but this effect is only local and has no global effect (i.e. effect on other participants' devices). Therefore we need to monitor independent devices and be able to do that in a coordinated fashion.

\vspace{5pt}\noindent\textbf{App Navigation.} In a lot of cases the analysis needs to happen through the mobile apps as this helps eradicate some challenges we face at the network level. An automated approach should be able to automatically navigate to a particular screen of interest of an app under analysis. This could be perform through a static or a dynamic execution approach. Static execution has the disadvantage that it can follow dead code paths (never invoked in practice). On the other hand dynamic execution might have coverage issues. However (1) most of these apps are designed to be simple and (2) to address the \textit{black box} limitations of the analysis we need to dynamically monitor server requests to specific triggers. For these reasons we chose a dynamic execution approach. Even then, our approach would require identifying user interface elements and their positioning within the screen, making a decision on which one should the tool interact with and then interact with it (click on it, click and input a number). Unfortunately a lot of elements have similar characteristics, which make automatic navigation challenging.

\subsection{Design Overview}
To tackle those challenges we designed \systemName{}, a \textcolor{semi-automated} modular framework which greatly facilitates the analysis of the resilience of ubiquitous crowdsourcing services. Figure~\ref{fig:arch} illustrates the overall architecture of \systemName{}.

\systemName{} consists of three main components: the coordinator node, the poisoning node and the observation node. The coordinator node takes as input a target apk (Android app executable) for analysis and a configuration file. The apk corresponds to the Android mobile app of the target service and the configuration file contains the choices of modules to enable. These can be specific to the target app and might require some manual preliminary analysis. \textcolor{red}{what kind of analysis/effort is required..explain...}. 

The coordinator's main role is to enable the required modules in the poisoning and observer nodes and coordinate their execution. This is crucial for obtaining reliable attack success rate results. For example, when analyzing \textit{Transit}, the injection node and observation nodes need to run the app on two different emulator devices. The app on the poisoning side will need to generate and fake an artificial bus ride on a specific route. The app on the observation device will need to request a route which overlaps with the poisoned one but commences later in space but at the same time. Moreover, the coordinator updates the observation node with whether the fake bus was created successfully and with the speed and location of the fake bus. This will allow the observation node to determine what should be the expected arrival time of the fake bus. The observation node uses this knowledge in tandem with its original expected arrival time, to determine whether the attack succeeded, i.e. whether there is a change in the expected arrival time which is a result of the fake bus. Moreover, the coordinator determines the evaluation plan and guides its execution. That is, it will decide based on the configuration properties, how many times an experiment should be repeated, what input type(s) should be examined and what value they should be assigned.

The poisoning node, executes the apk from the perspective of the adversary, using the configuration properties and values provided by the coordinator. The poisoning node can inject values directly through the \textit{network} or through the mobile app. In the latter case, the poisoning node can either spoof UI inputs or sensory inputs. For UI spoofing, it leverages \textit{dynamic execution} to drive the app to a target data poisoning screen, identify the input field of interest and fake a user input. For sensory input spoofing, the poisoning node generates a time series with the fake sensor values which feeds through API instrumentation to the mobile app at a speed determined by the coordinator and controlled by the poisoning node.

The observation node, executes the apk from the perspective of other users of the service. Its role is to identify whether the fake data injected by the poisoning node, has an effect on other users (and in essence accepted and used by the service). It executes the apk on a number of devices ($1..n$), and uses similar techniques with the poisoning node to monitor the execution of the app. For example, the observation node monitors the network traffic for \textcolor{red}{Ancestry.com} to determine whether the service is responding to fake requests and to determine the content of the service's responses. It can also use \textit{dynamic execution} to navigate to specific target screens. The observation node, further employs image classification techniques for dynamically analyzing the user interface of the victim user(s).

Next we elaborate on the most important modules supported by \systemName{}, in particular the \textit{network traffic} module, the \textit{dynamic execution} module, and the \textit{UI Analysis} module. 

\subsection{Framework Analysis Modules}

\vspace{5pt}\noindent\textbf{Network Traffic Module.} 
The network traffic module consists of a man-in-the-middle proxy between the observer or poisoning node and the network gateway. The nodes that use it download and install a CA certificate from the proxy. Normally this would have had been enough to enable observing the target apps traffic in plaintext but some apps are using mitigation strategies against MITM attempts and in particular a technique called certificate pinning. This configures the client app to accept connections only with the legitimate server. Thus the app under analysis would reject the proxy certificate trivially provided by our system. To address this, \systemName{} uses dynamic instrumentation which targets and overloads the ssl context initialization function (\textcolor{red}{name the funcions explicitly}) of the target app at runtime so that it uses the proxy's certificate and effectively bypassing the app's certificate pinning. This allows the MITM proxy to collect the network requests made by the target app when a value is injected and the responses by the crowdsourcing service. The proxy can be configured to send any number or kind of network requests to a server API and monitor the response to each request. Our current implementation uses an extended version of the Android Frida framework~\cite{} to facilitate the dynamic instrumentation.

%The network traffic module works as follows: First we run a man-in-the-middle proxy on our computer. Then, we install a certificate authority certificate corresponding to this man-in-the-middle proxy on our phone and set this proxy on the phone. Normally, this would have had been enough to observe the target apps traffic but recently apps have started using a new defense known as the certificate pinning defense where they do not trust certificates provided by the system and hence our installed certificate would not work and now we will have to break this defense too. 

%So, we put the frida binary on the phone which is a dynamic instrumentation framework and a script that this framework will use to overload the ssl context initialization function of our target app so that it starts using the certificate authority certificate provided by us thereby bypassing certificate pinning. 

%Now, we run the frida binary on the phone and use it to launch our target app with the overloading script. Now, we can start observing the https network traffic on our man-in-the-middle proxy. 

%We now interact with the app on the phone while observing network requests relevant to us and note them down. Next, we create a python script using the requests module to imitate the requests we had seen and noted down. So, in this way we reverse engineer the api of the app and then use the api to inject fake data into the app's servers.


\vspace{5pt}\noindent\textbf{Dynamic Execution Module.} 
%\textcolor{red}{Sojhal: please describe how does this work. You can use one of the apps as a running example.} Some accuracy analysis/evaluation would help here.
%\textcolor{red}{Make sure to mention how we handle similar IDs and classes and other execution challenges}
The Dynamic Execution Module (DEM) is a semi-automated UI interaction record and replay module. Android apps have a number of basic components: Services (functions executed in the background); content providers (for storing and retrieving data); Broadcast Receivers (callback functions for notifying the application for major system events); and Activities (foreground functionality). Activities are responsible for rendering a user interface on the screen. These interfaces are commonly declared statically at development time in layout files using an extensible markup language (XML). Less commonly, developers add, remove or manipulate elements programmatically. Each UI element, whether declared statically or programmatically can be associated with an element ID. The DEM module can monitor the IDs of UI elements the user interacts with during recording. When an app's layout is dynamically rendered, the DEM recorder parses the hierarchy tree of the layout and with the help of the analyst identifies the IDs corresponding to the UI elements of interest.  Note that it is not mandatory for UI elements to have IDs or even if they do they are not necessarily unique. To address this, the DEM also records auxiliary information related to the UI element of interest such as its position within the hierarchy tree, the element's class, and any textual information (e.g. strings associated with text labels of the element) semantically describing the element. During replay, the DEM leverages the android debug bridge to install and launch the app under analysis on an emulator or real device according to the configuration. It then uses the recorded UI elements' information and their logical order of execution to generate UI interaction commands sent through \texttt{adb} to the app. Like before, if there is a conflict of IDs or absence of them, the DEM replay looks for semantic hints using regular expressions or exact matching on strings, class names and position within the hierarchy tree to determine which element to emulate an interaction with. Our current implementation uses extended versions of the Android UIAutomator~\cite{} during recording and the appium framework~\cite{} during replay.

%For recording we use the Android UI Automator and for replay the Appium driver.
%When enabled, it makes use of a UI interaction tracking tool which records the UI layout class=
%makes use of a UI Monitor tool, and a UI driver tool. It can facilitate tracking UI interactions and replaying 
%The dynamic execution module works as follows: First, we make sure that an attack phone is connected to our computer and that adb is working on the phone. Then, we install our target app on the phone and launch it. Next, we launch the uiautomatorviewer2 tool on our computer which is user interface analyzing tool and helps view the ids and classes of elements on the screen. We trace a path to the screen where data injection or observation will happen and keep noting the ids and classes of the elements we would have to interact with this on path to do our intended action of data injection or observation. 
%Next, we use the appium framework to automate actions on the this phone to automatically do the injection or observation as a normal human would do if he interacts with the phone. For this, we first write a python script which leverages the ids and classes of elements we noted earlier on various screens on the path to our target action of injection or observation. Next, we launch the appium server on our computer followed by deploying the python script we just wrote. The appium server takes the actions from python script and passes them to the phone attached to the computer via adb thus automating the injection and observation process. 
%Note, that this process involves some challenges such as not all elements found on different screens have unique ids or ids at all. In such a case, we use the class of the element in combination with the text present on the element using regular expressions or exact matching. 

  \vspace{5pt}\noindent\textbf{UI Analysis.\textcolor{blue}{(TBC)}}
For some apps, their analysis might require looking into visual cues in their user interface. For example, the \textit{Transit} app uses an icon on the screen to provide real-time feedback to its users about the movement of selected public buses on a target route. Identifying the bus visual cues would allow us to automatically determine whether an attack was successful in creating a fake bus ride. However, it might be the case that the fake bus ride did not actually affect the estimated time of arrival (ETA) of a bus on a victim user's screen. This can further be verified by extracting the ETA from observer nodes. In other words, for \textit{Transit}, determining the success of the attack would require identifying the bus and its movement on the UI screen of the poisoning node, in conjunction with a semantically meaningful change in the expected arrival time for that bus captured on the UI of the observer node.

The UI Analysis module can facilitate recognition of visual elements in a user interface. The nodes are responsible for providing RGB screenshots of the UI needs analysing and for selecting a mode of operation. Currently the UI Analysis module supports two modes: icon recognition and text detection. Icon recognition, expects as additional input, the icon to search for. This can be easily extracted by decompiling the target app (e.g. with the apktool~\cite{}) and looking into its \texttt{res/drawable} folders for the icon.  It then uses the \texttt{MatchTemplate()} function of the openCV2 library (Open Source Computer Vision Library) to search the sample image within a grayscale version of the provided screenshot. 
%\texttt{MatchTemplate()} can be tuned in different levels of sensitivity using a threshold value. This controls how many of the pixel RGB values in an area of interest should match the sample icon.  We set the threshold to 90\%.. 
In text detection mode, the module expects a string, and a region of interest boundary as additional inputs to the screenshot. It then converts the given RGB matrix of the screenshot into grayscale, and performs optical character recognition (OCR) in the region of interest. In our implementation we used the \texttt{pytessseract} Python library for OCR.   

%UI Analysis, which contains two parts: text recognition and icon recognition, allows us to do realtime observation based on computer vision . The text recognition takes grey images which are converted from RGB screenshots as inputs. Using pytesseract which is an optical character recognition (OCR) tool for python, the interested parts of grey images are converted to string format. In icon recognition, openCV2 (Open Source Computer Vision Library) is used to match and recognize specific icons on grey images.

%To achieve this, we first decompiled the target app to acquire the sample icons. Then the openCV2 calls MatchTemplate() to search the sample icon within grey images. Once the similarity is over 90\%, MatchTemplate would output the position of the recognized icon. Taking Transit as an example, text recognition allows us to track the expected waiting time while icon recognition allows us to track the adversarial bus appeared on the victim screen. In this way, we can confirm whether our attack is successful and how much has our attack influenced other users.
%\textcolor{red}{Comment: Can we also describe how those libraries do this (how pytesseract does ocr; how does opencv2 identifies icons)? Even though we did not develop those algorithms, we need to show understanding of the internals of how they work. This will help us explain better how the UI Analysis module works precicely. Accuracy analysis/evaluation at the Framework evaluation section.}

\vspace{5pt}\noindent\textbf{Sensor Spoofing Module.}
Some apps require sensor spoofing to perform successful data poisoning. For example \textit{Neighbors by Ring} reads and reports the GPS coordinates whenever a new event is posted. \textit{Transit}, during a bus ride, continuously reports the GPS coordinates of the host device. The sensor spoofing module can be configured to provide fake device GPS readings (longitude and latitude) to a device (either a real device or an emulator). It can be configured in static and dynamic mode. In static mode, it fixes the GPS coordinates of the device to a pre-specified longitude, latitude pair. In dynamic mode, it keeps changing the device's location using a provided timeseries of GPS values. The dynamic mode was used to control the speed and location of the device when analysing \textit{Transit}. \textcolor{red}{Charles: how is this implemented? What commands did we use to inject/change the GPS location of the emulator? Does the emulator need to be rooted? Does it need to have mock location enabled? Please provide details.} \textcolor{blue}{By using Genymotion Shell commands, we are able to activate the GPS through\textit{ gps setstatus enabled} and set our own locations on the unrooted emulator through  \textit{gps setlatitude} and \textit{gps setlongitude}. Based on that, the moving speed is controlled by the time delay of injecting each fake location. }

%\textcolor{red}{Charles:}
%Sensor-based apps use different sensors to achieve various functionalities such as tracking movements and monitoring heartbeat. Sensor spoofing module first accesses the permission to manipulate the data of each sensor. For instance, to change the position of the Transit user, we need the permission to change the GPS data. Then, to be effective, this module mimics the characteristic of the real data so that the generated data is reasonable. For example, when generating fake buses, buses with reasonable movements are accepted by the app while buses with unreasonable movements such as at very high speeds or out of roads would not be accepted but regarded as abnormality. After that, the injector node feeds the fake sensor values along with a time series to the target app at a speed determined by the coordinator.   

%Our analysis on Section~\ref{sec:threats} shows that attacks can manifest due to context
\ignore{
% embed in experiment design for each app
\subsection{Input Domain Range Exploration Strategies.}

\subsubsection{GPS.}

\subsubsection{Integer.}

\subsubsection{Float Point.}

\subsection{Semantics Exploration Strategies.}
\subsubsection{Firstname.}

\subsubsection{Hazardous event descriptions.}

\subsubsection{Speed.}

\subsubsection{Location.}

\subsubsection{Time.}
}

%Integers: the set of positive numbers $\in \mathbb{Z}$.

%Float Numbers: $\in \mathbb{R}$

%String: 




==> old_framework/4_evaluation.tex <==
%EVALUATION OF FRAMEWORK COMPONENTS


\subsection{Dynamic Execution.}
\textcolor{red}{What to measure?
For each of our apps use UI Analyzer to go to injection screen.
For each  one use dynamic execution server 100 times and measure (1) how many times out of 100 the dynamic execution server resulted in navigating to the right screen and (2) how long did it take.}

\subsection{UI AnAlysis.\textcolor{blue}{(TBC)}}
\textcolor{red}{Icon finder, ocr, final icon finder+ocr alorithm accuracy and time. What else?}

\subsection{end to end system.}
\textcolor{red}{create ground truth for input domain experiments. This means run XX experiments for XX apps and manually check how many times and with what experiment configuration the attack is successful or failed. Label each experiment. This is the ground truth. Then repeat the same experiments using the automated framework. Check the framework's decision (attack succeeded or attack failed and compare with ground truth). Report on false positives and false negatives.}



==> old_framework/5_characterisation.tex <==
% ATTACK EXPERIMENTS - CHARACTERISATION
%Characterization of Attack Surface of Ubiquitous Crowdsourcing Services
We leveraged our framework (see Section~\ref{sec:framework}) to perform a number of experiments to help us systematically characterize an adversary's data poisoning capabilities against all mobile crowd-sourcing services listed in Table~\ref{tab:inputTypes} . 

In particular we aim to answer the following research questions:
\begin{itemize}
    \item \textit{RQ1.} What is the range of the input domains of mobile crowd-sourcing services. %Input Domain Poisoning Range.
    \item \textit{RQ2.} To what extend is semantic validation applied by mobile crowd-sourcing services.
\end{itemize}


%\subsection{Experiment Setup}
%Implementation details: what tools did we use (mallory, wireshark, in what topology; emulator vs real phones, one for injection , one for monitoring, laptop/desktop as coordinator, appium for tracking ui elements, UI analyzer for? what else?? Please describe the setup)

%Evaluation plan:
%Then, for which apps, which components of the framework did we use; what did we measure (how are the experiments designed) (input domain (see Table~\ref{tab:inputTypes}), context (time, location)).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiments.}
To answer our research questions, for each MCS, we design appropriate input generation strategies according to the UI and sensory input types their companion mobile apps support or by directly spoofing their API requests when possible.

\subsubsection{Ancestry.com}
\vspace{5pt}\noindent\textbf{Experiment Design.}
\textit{Ancestry.com} allows their users to search for people in their database. In Section~\ref{sec:threats} we discussed our manual attack. With the help of our framework, we designed and conducted two experiments to measure the extend of the problem. 

This service allows users to search individuals' records using a record ID. It accepts that through the user interface as an integer value. \textcolor{red}{Explain experiment.}


The service also allows searching records using names. Users can input the name to search for as a string value in the app's UI. \textcolor{red}{Explain experiment.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{MyHeritage}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Transit}
\vspace{5pt}\noindent\textbf{Experiment Design.}

To analyse the transit app, we use the sensor spoofing module as mentioned in 3.4. Three experiments were performed during off peak time in rural area of London: \\
1. Allowed adversarial speed.\\
By changing the speed of injecting fake locations, we are able to change the speed of the emulator and find the speed boundary within which the transit would accept the emulator as an active bus rider. Based on that, 50 speed values within the speed boundary are chosen to further show the speed acceptance rate, as shown in table 1.\\
2. Adversarial speed Influence on expected waiting time. \\
By using the same speed within the speed boundary, an attack emulator is used to fool transit as if it has got on the coming bus. Then, the speed is ranged from 0 to 200km/h continuously generating fake routes. At the same time, an observation emulator waited for the same bus at certain stops further than the attacker and recorded the waiting time change for each attack speed. The results are shown in fig 1.\\
3.Adversarial distance Influence on expected waiting time. \\
By using the same speed within the speed boundary, an attack emulator is used to fool transit as if it has got on the coming bus. Then, the attack distance from the victim emulator is ranged from xx to xx continuously generating fake routes. At the same time, the victim emulator waited for the same bus at the same location and recorded the waiting time change for each attack distance. The results are shown in fig 1.\\
\vspace{5pt}\noindent\textbf{Results.}
As shown in table 1, the speed boundary is [XX,XX]. Within this boundary, all 50 speeds were accepted by transit.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Neighbors by Ring}
\vspace{5pt}\noindent\textbf{Experiment Design.} In this set of experiments, we aim to evaluate the natural language understanding performed by the app. We submit posts, text only, at different level of coherence and relevance to the app and take note of how many of them get accepted. For the ones that do not get through, we submit them again with a relevant picture and record the outcomes. For posts of type crime, safety or unexpected activity we upload a picture of a hooded man and for lost pets we use a picture of a dog.
In order to generate text, we use the pre-trained model GPT-2, a state-of-the-art Transformer-based model []. We generate each type of posts by using keywords, selected from existing users' posts, as prompts for the model to complete. Text directly generated from the model might be semantically sound but is not relevant to the type and format of content the app requires, thus represent our simpler level of semantics. 
The second experiment tests more relevant posts generated by fine-tuning the model on 1080 submissions collected through the app. The prompts given to the model now become the type of posts that is to be generated. Again, we take note of the acceptance rate with and without a picture.         


\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Basket Savings}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Gus Buddy}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Police Detector}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Public Toilet}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Map My Run}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Strava}
\vspace{5pt}\noindent\textbf{Experiment Design.}
For each of the activities running, cycling and swimming, the fake json data with different activity information such as exercising dates, distance, time and descriptions  is generated and posted . Command \textit{requests.post} on \textit{https://m.strava.com/api/v3/activities} is used to post whereas command \textit{requests.get} on \textit{https://m.strava.com/api/v3/athletes/userID/stats} is used to check Whether the injection has been accepted. All experiments are done with one user account  with a unique userID allocated by the API) .\\
Focusing on two main  moving parameters including time and distance, we consecutively post fake activities to find the single and total injection boundary , as shown in table 3 and table 4.  We also see how many consecutive posts we can add in a day, as shown in table 5.\\
\vspace{5pt}\noindent\textbf{Results.}
As shown in table 3 and table 4, all three exercise types share the same boundary and only accept positive integers. Both single injection and total injection have the same maximum time 31,622,400 seconds which is also 366 days. The maximum acceptable distance of single injection is 50,000,000 miles which would definitely reach the top one on any club leaderboard. For the total injection, the maximum acceptable distance is 4,294,967,295 miles which is right the same with the maximum range of unsigned integer data type. Table 5 shows that the maximum number of posts can be accepted by strava is 50 for every picked date. If we want to inject more posts, it is necessary to change the picked date. 
\begin{table*}[]
\centering
\caption{Strava experiments: single injection}
\label{tab:inputTypes}
\begin{tabular}{| c | c | c | c | c | c| } \hline
  Num& Type          & \multicolumn{2}{c |}{Time(second)} & \multicolumn{2}{c |}{Distance(mile)} \\ \cline{3-6}
   &          & max & min & max&min \\ \hline
1 & Run  & 31,622,400 & 0 & 50,000,000 & 0 \\
2 & Ride & 31,622,400 & 0 & 50,000,000 & 0 \\
3 & Swim& 31,622,400 & 0 & 50,000,000 &0 \\ \hline
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\caption{Strava experiments: Total injection}
\label{tab:inputTypes}
\begin{tabular}{| c | c | c | c | c | c| } \hline
  Num& Type          & \multicolumn{2}{c |}{Time(second)} & \multicolumn{2}{c |}{Distance(mile)} \\ \cline{3-6}
   &          & max & min & max&min \\ \hline
1 & Run  & 31,622,400  & 0 & 4,294,967,295 & 0 \\
2 & Ride & 31,622,400 & 0 & 4,294,967,295 & 0 \\
3 & Swim& 31,622,400 & 0 & 4,294,967,295 &0 \\ \hline
\end{tabular}
\end{table*}


\begin{table*}[]
\centering
\caption{Strava experiments: consecutive posts allowed to be added in a day}
\label{tab:inputTypes}
\begin{tabular}{| c| c | c | c | c | c | c| } \hline
 Num& Date& run&ride&swim & total  \\ \hline
1 & 27/3/2020  & 19 & 19 & 12 & 50 \\
2 & 28/3/2020  & 50 & 0   &  0  & 50 \\
3 & 29/3/2020  & 46 & 0   &  4  & 50 \\ 
4 & 30/3/2020  & 0   & 50 &  0  & 50 \\
5 & 31/3/2020  & 0   & 0   & 50 & 50 \\
6 & 31/3/2020  & 48 & 0   & 2   & 50 \\ 
\hline
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Fitbit}
\vspace{5pt}\noindent\textbf{Experiment Design.}

\vspace{5pt}\noindent\textbf{Results.}



\subsection{Main Sources of anomalies.}
Discuss (group) analyses findings. For example, (1) erroneous threat model - ancestry returns all values to client free/paid and filters at the client. (2) impossible and semantically anomalous values: really long runs map my run 151K miles, really fast speed for bus; semantically anomalous - toilet in ocean , prices too low for market

\subsubsection{RQ1. Input Domain Range Validation.}
Integers, floats.

\subsubsection{RQ2. Input Semantic Validation.}
When looking at semantics we foudn that...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\subsection{Characterization Results}

\subsection{Characterization Results}
general techniques, what can it be achieved.
Maybe separate per input type/time of day pairs.

\subsubsection{Transit Experiment Results}

\subsubsection{Neighbors by Ring Experiment Results}

\subsubsection{Ancenstry.com Experiment Results}

\subsubsection{MyHeritage Experiment Results}

\subsubsection{Basket Savings Experiment Results}

\subsubsection{Gus Buddy Experiment Results}

\subsubsection{Police Detector Experiment Results}

\subsubsection{Public Toilet Experiment Results}

\subsubsection{Map My Run Experiment Results}

\subsubsection{Strava Experiment Results}

\subsubsection{Fitbit Experiment Results}
}

==> old_framework/7_discussion.tex <==
% DISCUSSION OF THREATS- reason and defense

==> old_framework/apps.tex <==
\section{Apps}
\label{sec:apps}

\subsection{Neighbors by Ring}
Neighbors is an app by Ring that allows its users to report crimes within their neighborhood and
upload photo and video evidence to warn the local community. Furthermore it gives incident
maps and crime reports in the form of bar graphs for the neighborhood to users.
The attack is to create confusion and chaos in the people of a neighborhood by posting a fake
crime/suspicious activity within the bounds of the neighborhood every few hours.
Alternatively, we can find out how many input posts and what kind of input posts are possible to
be sent to the app by fuzzing the input space of the app.

\subsection{Basket Savings}
Basket is an app which crowdsources prices of similar items on different stores so that
customers can both share prices for items and get the best price for any item present at multiple
stores.
The attack is to increase or decrease customers to a particular store by increasing or
decreasing prices of a list of most popular grocery items significantly.
Alternatively, we can find out how much the prices can be altered by fuzzing the inputs.

\begin{table}[]
\centering
\caption{Basket: Trader joe's}
\begin{tabular}{llll}
Product                           & Value & Min & Max \\
Apples                           & 0.49 & 0.05 & 2.0 \\
Bananas        & 0.19 & 0.09 & 2.0 \\
Strawberries        & 0.99 & 0.09 & 2.0 \\
Eggs                 & 1.99 & 0.2  & 4.0 \\
Chicken Breasts     & 2.69 & 0.27 & 6.0 \\
Organic whole Milk & 3.49 & 0.35 & 8.0
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Basket: Amazon Prime}
\begin{tabular}{llll}
Product                           & Value & Min & Max \\
Apples             & 1.58 & 0.16 & 4.0 \\
Bananas            & 0.55 & 0.06 & 2.0 \\
Strawberries       & 5.0  & 2.21 & 8.3 \\
Eggs               & 2.12 & 0.21 & 6.0 \\
Chicken Breasts    & 3.25 & 0.33 & 8.0 \\
Organic whole Milk & 3.76 & 0.38 & 8.0
\end{tabular}
\end{table}

\subsection{GasBuddy: Find Cheap Gas Prices \&amp; Fuel Savings}
Similar to basket, gasBuddy is a crowdsourcing platform for comparing prices of gas at different
gas stations. They get their data from their users who report price changes for gas at any
particular gas station.
The attack is to increase or decrease cars to a particular gas station by increasing or decreasing
prices of gas significantly.
Alternatively, we can find out how much the gas prices can be altered by fuzzing the inputs.

\subsection{Public Toilet App}
Public toilet app is a crowdsourcing app that allows users to find public restrooms in time of
need. It also has an option for the community to help by adding new public toilets or
editing/removing previous public toilets.
The attack involves adding fake toilets to some regions in order to attract people to come there
and once they are at a place, they can be scammed or looted. Some one can also delete legit
public toilets from the app so as to reserve the public toilet just for themselves.
We can also find out how many fake toilets can be added to a region or how many legit toilets
can be deleted by a malicious user.

\subsection{Police Detector (Speed Camera Radar)}
Police detector is a crowdsourcing app that uses crowdsourcing to help users make intelligent
decisions while driving and get to their destinations faster. It lets users see the police detectors,
road repairs and road accidents on any current road. It also allows the users to add these
police detectors, road repairs and road accidents on any current road.
This can be attacked by adding fake aforementioned items on some particular road to block
users away from it. Some homeowners can do this on roads of their neighborhood to keep it

traffic free or some malicious user can do that to reduce his commute time by diverting other
vehicles to alternate roads by placing these fake deterrents on roads. Also some one can delete
legit items from roads to get people frustrated.
We can also find out how many fake objects can be added to a region on the map or how many
legit objects can be deleted by a malicious user from the map.

\subsection{Run with Map My Run}
This is a fitness app that helps people who want to run. It provides multiple features to keep its
users motivated to run like actively posting challenges and letting the users publish their runs to
their walls to boast of to their friends. Also, note that some challenges are sponsored and
involve real rewards too.
The attack involves adding fake runs to the app by a user to win these challenges or fool your
online friends without actually ever moving.
Furthermore, we can study how many runs and how much odd runs can a user add.

\subsection{MyHeritage - Family tree, DNA \&amp; ancestry search}
This app lets you build your family tree, search people through their data-set and get automatic
suggestions(paid) for family tree matches. Also, you can order DNA Kits and get detailed
analysis of your dna through them.
The app also has a feature to search through their database. We intend to exploit this feature
and download their database.

\subsection{Ancestry.com}
This app lets you build your family tree, search people through their data-set and get automatic
suggestions(paid) for family tree matches. Also, you can order DNA Kits and get detailed
analysis of your dna through them. Additionally, you can send any member messages too. This
can be used for elaborate scams. The members you can search and family tree suggestions
only come from data records like electoral records or marriage histories but you can access the
ancestry.com records by paying the membership fee.
The app also has a feature to search through their database. We intend to exploit this feature
and download their database.

\begin{table}[]
\centering
\caption{Ancestry: Attack1 All Fields}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Name & 9998 \\ \hline
Gender & 351 \\ \hline
Notes & 10000 \\ \hline
Father & 94 \\ \hline
Birth Place & 5327 \\ \hline
SSN & 10000 \\ \hline
Mother & 94 \\ \hline
Death Date & 3044 \\ \hline
Claim Date & 9716 \\ \hline
Birth Date & 9999 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Ancestry: Attack1 Veiled Fields}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Gender & 342 \\ \hline
Claim Date & 9339 \\ \hline
Father & 89 \\ \hline
Birth Place & 3896 \\ \hline
SSN & 9611 \\ \hline
Mother & 88 \\ \hline
Death Date & 2916 \\ \hline
Notes & 9611 \\ \hline
Birth Date & 9610 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Ancestry: Attack1 Record Categories}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Court, Governmental & Criminal Records & 10000 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Ancestry: Attack2 All Fields}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Death & 166 \\ \hline
Father & 172820 \\ \hline
Spouse Residence & 3 \\ \hline
Vital & 172846 \\ \hline
Arrival & 35 \\ \hline
Parent & 3 \\ \hline
Birth & 922177 \\ \hline
Spouse & 1613376 \\ \hline
Spouse Birth Year & 57611 \\ \hline
Bond date & 7 \\ \hline
Name & 5761498 \\ \hline
Widow's Death Place & 1 \\ \hline
Residence & 453 \\ \hline
Departure & 7 \\ \hline
Spouse Residence Place & 20 \\ \hline
Marriage & 3168821 \\ \hline
Spouse Birth Place & 57611 \\ \hline
Mother & 57608 \\ \hline
Military & 1 \\ \hline
Origin & 3 \\ \hline
Date Discharged & 1 \\ \hline
Civil & 4 \\ \hline
Widow's Death Date & 1 \\ \hline
Relative & 36 \\ \hline
Sibling & 4 \\ \hline
Bond Place & 7 \\ \hline
Spouse Birth Location & 2 \\ \hline
Children & 23 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Ancestry: Attack2 Veiled Fields}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
Arrival & 12 \\ \hline
Origin & 1 \\ \hline
Death & 140 \\ \hline
Bond date & 7 \\ \hline
Parent & 2 \\ \hline
Sibling & 4 \\ \hline
Residence & 377 \\ \hline
Father & 164852 \\ \hline
Departure & 1 \\ \hline
Spouse Residence Place & 20 \\ \hline
Relative & 6 \\ \hline
Spouse Residence & 3 \\ \hline
Vital & 164879 \\ \hline
Marriage & 3022626 \\ \hline
Spouse Birth Place & 1 \\ \hline
Birth & 879587 \\ \hline
Mother & 54951 \\ \hline
Spouse Birth Year & 54956 \\ \hline
Children & 21 \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Ancestry: Attack2 Record Categories}
\label{tab:inputTypes}
\begin{tabular}{| l | l |}
 Fields          &  Times Found \\ \hline
1900s (Decade) & 24 \\ \hline
Birth, Baptism \& Christening & 115356 \\ \hline
Draft, Enlistment and Service & 41 \\ \hline
1830s & 4 \\ \hline
Passenger Lists & 10 \\ \hline
1880s & 3 \\ \hline
1940s & 14 \\ \hline
1920s & 141 \\ \hline
Soldier, Veteran \& Prisoner Rolls \& Lists & 7 \\ \hline
Citizenship Records & 21 \\ \hline
1850s & 2 \\ \hline
1930s & 70 \\ \hline
1870s & 9 \\ \hline
1860s & 6 \\ \hline
Death, Burial, Cemetery \& Obituaries & 241 \\ \hline
Marriage \& Divorce & 5645501 \\ \hline
Pension Records & 2 \\ \hline
Court, Governmental \& Criminal Records & 10 \\ \hline
1910s & 34 \\ \hline
1840s & 3 \\ \hline
\end{tabular}
\end{table}

\subsection{Transit}
Transit is a navigation app for public transport. It helps users choose the best public transport
route that will take them to their destination in the shortest time by the help of crowdsourcing
data from their users to track where a public transport bus or train is right now.
The attack involves misguiding users and making them choose the wrong routes by simulating
fake online movement of certain buses.
We can also explore how many users and what kind of input is needed to fool the app’s system.

\subsection{Strava: Track Running, Cycling \& Swimming}
Strava is an app tracking your running, cycling or swimming . Your speed, length, time are
recorded. You can share your routine with your friends and see the ranking among your friends.

You are able to join different kinds of clubs and compete with other people. Your achievements
will appear on the leaderboard if you are one of the top 100.
The attack involves adding fake activities to the app by a user to come to the top of a
leaderboard, win badges or fool your online friends without actually ever moving.
Furthermore, we can study how many activities and how much odd activities can a user add.

\subsection{Fitbit app}
Fitbit is a fitness app recording your all-day activity. For activity, it can record walk, Hike and
Run. You can share your achievements with people in different groups and earn badges and
participate in challenges.
The attack involves adding fake activities to the app by a user to win these challenges or fool
your online friends without actually ever moving.
Furthermore, we can study how many runs and how much odd runs can a user add.



==> old_framework/attack.tex <==
\section{Attacks}
\label{sec:attacks}
This section describes the attacks on apps:

%-----------------------------------------------------------------------------
\subsection*{Neighbors by Ring}
Neighbors is an app by Ring that allows its users to report crimes within their neighborhood and upload photo and video evidence to warn the local community. Furthermore it gives incident maps and crime reports in the form of bar graphs for the neighborhood to users.
 
We attacked this app by posting fake posts to the neighborhood. Some of the posts went through while some didn’t. They might have employed a machine learning model to determine if a post is legit.
 
For instance, these posts got rejected:
“dangerous cat spotted near tree”
“dangerous donkey spotted”
“Saw phone getting mugged nearby.”
 
While, these posts went through:
“Dangerous dog wandering around went through”
“mugging phone on 35th street”  with fake case number and agency number in crime section. Note that 35th street is a fake street.



\begin{itemize}
    \item \textbf{Goal: } Incident/event report (SAFETY)
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item alarm users, cause fear, waste resources
            \item Temporal: real-time
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject unstructured text + optional case number + optional agency number
            \item USER INPUT (attack on UI) 
            \item through normal functionality of victim app
            \item min number of adversarial nodes required: single
        \end{itemize}

    \item \textbf{Challenges: } avoiding their filtering system,  not harming people. Experiments were done very late at night and were immediately reverted after the attack was verified.
        

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Basket Savings}
Basket is an app which crowdsources prices of similar items on different stores so that customers can both share prices for items and get the best price for any item present at multiple stores. The default option for storing prices is to scan barcodes of given items using the app and you can only do this while you are at the location of the store. However, we perform the attack by exploiting an edge case where the app allows you to add price for a given item if you are at home and the receipt has no barcode. We increment the price of apples by 1 cent at target and the change is propagated to other phones too. We change it back to original price as soon as we validate the attack has been successful.



\begin{itemize}
    \item \textbf{Goal: } Price report (PRICING) 
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item drive users to different provider, confusion, fake data 
            \item Temporal: real-time
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject number (text) for target item
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single
            
        \end{itemize}

    \item \textbf{Challenges: } not harming people. Experiments were done very late at night and were immediately reverted after the attack was verified.

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{GasBuddy: Find Cheap Gas Prices \& Fuel Savings}
Similar to basket, gasBuddy is a platform for comparing prices of gas at different gas stations. They get their data from their users who report price changes for gas at any particular gas station. We attack this app in a similar fashion to the basket app by suggesting 1 cent increase in gas price on a nearby gas-station. We validate the change in price on other phones and then quickly revert the change back.



\begin{itemize}
    \item \textbf{Goal: } change price of item (PRICING) 
        
    \item \textbf{Outcome: } 
        \begin{itemize}
            \item drive users to different provider, confusion, fake data 
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject number (text) for target item 
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single
        \end{itemize}

    \item \textbf{Challenges: } not harming people. Experiments were done very late at night and were immediately reverted after the attack was verified.
        
\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Public Toilet App}
Public toilet app is a crowdsourcing app that allows users to find public restrooms in time of need. It also has an option for the community to help by adding new public toilets or editing/removing previous public toilets. The attack involves adding fake toilets to some regions in order to attract people to come there and once they are at a place, they can be scammed or looted. Some one can also delete legit public toilets from the app so as to reserve the public toilet just for themselves.



\begin{itemize}
    \item \textbf{Goal: } Add fake toilets. Remove legit public toilets.
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Shopkeepers nearby can remove public toilets to reserve them for their use only. People can also add fake toilets to bring people to some secluded area for scams or malicious intent like mugging or looting. 
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject fake toilet location or delete legit public toilet
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single
            
        \end{itemize}

    \item \textbf{Challenges: } not harming people. Experiments were done very late at night and were immediately reverted after the attack was verified.
        

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Police Detector (Speed Camera Radar)}
Police detector is an app that uses crowdsourcing to help users make intelligent decisions while driving and get to their destinations faster. It lets users see the police detectors, road repairs and road accidents on any current road. It also allows the users to add these  police detectors, road repairs and road accidents on any current road. This can be attacked by adding fake aforementioned items on some particular road to block users away from it. Some homeowners can do this on roads of their neighborhood to keep it traffic free or some malicious user can do that to reduce his commute time by diverting other vehicles to alternate roads by placing these fake deterrents on roads. Also some one can delete legit items from roads to get people frustrated.



\begin{itemize}
    \item \textbf{Goal: } Adding fake police detectors, road repairs, road accidents on road, deleting legit detectors, repairs and accidents from road

        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Divert users from some roads. Attract people to use an alternative road more. Making people frustrated by deleting repairs from roads and getting people stuck on those roads.
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item Spoof fake location, inject police detector or remove police detector on spoofed location
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single
            
        \end{itemize}

    \item \textbf{Challenges: } spoofing location to add police detector, can be done by using a spoofing app and allowing the app to spoof location from developer settings.  Not harming people. Experiments were done very late at night and were immediately reverted after the attack was verified.

        

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Run with Map My Run}
This is a fitness app that helps people who want to run. The features of this app that can be attacked are the functionality to see other people’s activities on public wall and to get free rewards without running by simulating fake runs.



\begin{itemize}
    \item \textbf{Goal: }  Fake winning challenges with rewards, get people personal data that they share on wall for everyone 
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Get rewards for free without running and fool friends about your accomplishments, collect people address information from their running track they share on wall for everyone
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item Spoofing user location and simulating fake runs
            \item Fake sensor input
            \item through normal functionality 
            \item min number of adversarial nodes required: single
            
        \end{itemize}

    \item \textbf{Challenges: }  attack doesn't work on emulators, spoofing location with real phones

\end{itemize}

\iffalse
%-----------------------------------------------------------------------------
\subsection*{MyHeritage - Family tree, DNA \& ancestry search}
This app lets you build your family tree, search people through their data-set and get automatic suggestions(paid) for family tree matches. Also, you can order DNA Kits and get detailed analysis of your dna through them.
The app also has a feature to search through their database.


\begin{itemize}
    \item \textbf{Goal: } Search their database.

        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Get the apps data
            \item Temporal: not real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject name (text) for target item 
            \item crawl results
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single

        \end{itemize}

    \item \textbf{Challenges: } For advanced features like seeing full search results = you have to pay for subscription.

        

\end{itemize}
\fi
%-----------------------------------------------------------------------------
\subsection*{Ancestry.com}
This app lets you build your family tree, search people through their data-set and get automatic suggestions(paid) for family tree matches. Also, you can order DNA Kits and get detailed analysis of your dna through them. Additionally, you can send any member messages too. This can be used for elaborate scams. The members you can search and family tree suggestions only come from data records like electoral records or marriage histories but you can access the ancestry.com records by paying the membership fee.
The app also has a feature to search through their database.




\begin{itemize}
    \item \textbf{Goal: } Search their database.

        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Get the apps data
            \item Temporal: not real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject name (text) for target item 
            \item crawl results
            \item USER INPUT (attack on UI) 
            \item through normal functionality 
            \item min number of adversarial nodes required: single

        \end{itemize}

    \item \textbf{Challenges: } For advanced features like seeing full search results = you have to pay for subscription.


\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Google Maps}
We tried attacking this app both manually via 10 phones and via emulators but were not successful. However, we can quote Simon Wrecket’s popular attack on google maps in berlin where he walks around with 99 phones in the middle of a not so busy road for about an hour to trick google into believing that the road is very busy with traffic. 
(https://www.washingtonpost.com/technology/2020/02/04/google-maps-simon-weckert/)



\begin{itemize}
    \item \textbf{Goal: } Add fake congestion on roads. Make stores look busy when in fact they are not busy.
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item to divert people from roads,  to deter customers from certain roads.
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item Walk around on an empty street with 99 phones for about an hour
            \item Attack on sensors
            \item Gps and carrier-based location
            \item through normal functionality 
            \item min number of adversarial nodes required: 99
            
        \end{itemize}

    \item \textbf{Challenges: } a lot of phones with carriers were used and still took google about an hour to respond. Need phones, phone numbers and google accounts. Google maps app api not easily reversible.
        

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Transit}
Transit is a positioning and navigation map in which you can search the real-time routine from the start point to the destination. It also shows the upcoming departure times for all nearby transit lines such as buses and trains. By starting “GO” mode, you will share your routine with other people and see how many people you are influencing.



\begin{itemize}
    \item \textbf{Goal: }  change predicted arrival time for public transport (NAVIGATION) 
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item confusion 
            \item Temporal: real-time
            
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item inject route with fake speeds + fake location 
            \item attack on SENSORS  
            \item gps 
            
        \end{itemize}

    \item \textbf{Challenges: } Simulating fake passengers via emulators.
        

\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Strava: Track Running, Cycling \& Swimming}
Strava is an app tracking your running, cycling or swimming . Your speed, length, time are recorded. You can share your routine with your friends and see the ranking among your friends. You are able to join different kinds of clubs and compete with other people. Your achievements will appear on the leaderboard if you are one of the top 100.



\begin{itemize}
    \item \textbf{Goal: } change the leaderboard ranking in transit club (SPORTS) , fool friends about your accomplishments
        
    \item \textbf{Outcome: } 
        \begin{itemize}
            \item Leaderboard ranking 
            \item Temporal: real-time
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item Join running clubs
            \item create manual entries  
            \item attack on DATABASE  (UI)
            
        \end{itemize}
        
\end{itemize}

%-----------------------------------------------------------------------------
\subsection*{Fitbit app}
Fitbit is a fitness app recording your all-day activity. For activity, it can record walk, Hike and Run. You can share your achievements with people in different groups



\begin{itemize}
    \item \textbf{Goal: } Create fake sports routine without devices (SPORTS) 
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item Fake movement including walk, Hike and Run
            \item Temporal: real-time
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item Move the GPS position of emulators
            \item Share with open groups
            \item attack on Sensors  
        \end{itemize}        

\end{itemize}

%-----------------------------------------------------------------------------
\iffalse
\subsection*{}



\begin{itemize}
    \item \textbf{Goal: }
        
    \item \textbf{Outcome: }
        \begin{itemize}
            \item 
        \end{itemize}

        \item \textbf{Attack method: }
        \begin{itemize}
            \item 
        \end{itemize}

    \item \textbf{Challenges}
        

\end{itemize}
\fi

%-----------------------------------------------------------------------------
\section{Transit}
\subsection{APP Description}
Transit is a positioning and navigation map in which you can search the real-time routine from the start point to the destination. It also shows the upcoming departure times for all nearby transit lines such as buses and trains. By starting “GO” mode, you will share your routine with other people and see how many people you are influencing.
\subsection{Attack Method}
Attack Goal: change predicted arrival time for public transport (NAVIGATION)
Attack Type: attack on SENSORS
Attack Details: 
1.Choose an off-peak bus in rural area
2.Choose 3 emulators: E1, E2, E3
3.E1 started from 3 stops further than E2 \& E3. E2 \& E3 stayed at the same stop 
4.Start the "GO" mode of E1, E2, E3
5.By moving the GPS position of E1 very fast ( similar to the bus speed ), E1 fooled the transit app as if it was on the bus. 
6.After E1 getting on the bus, slow down the speed of E1 (nearly stop). A fake bus appeared on the screen of E2 and E3. 
7.By changing the speed of E1, the fake bus shown on the screen of E2 and E3 moved accordingly. Also, the expected waiting time of E2 and E3 changed according to the speed of E1.
Attack Challenges:Choose right time to avoid competition with too much real data

\section{Fitbit}
\subsection{APP Description}
Fitbit is a fitness app recording your all-day activity. For activity, it can record walk, Hike and Run. You can share your achievements with people in different groups.
\subsection{Attack Method}
Attack Goal: Create fake sports routine without devices (SPORTS)
Attack Type: attack on SENSORS
Attack Details: 
1.Moved the GPS position of emulator at a very fast speed(nearly 2km/s)
2.created fake activities including Walk, Hike and Run. The system commented on the created activities: Fastest hike ever.
3.share with open groups

\section{Strava: Track Running, Cycling \& Swimming}
\subsection{APP Description}
Strava is an app tracking your running, cycling or swimming . Your speed, length, time are recorded. You can share your routine with your friends and see the ranking among your friends. You are able to join different kinds of clubs and compete with other people. Your achievements will appear on the leaderboard if you are one of the top 100.
\subsection{Attack Method}
Attack Goal: change the leaderboard ranking in strava club (SPORTS) 
Attack Type: attack on UI
Attack Details: 
1.Join running clubs
2.create manual entries which contains distance, duration, elevation and sport type.
3.The fake activity ranked first on the learderboard. It was also flagged by other people.
Attack Challenges: It seems Strava can recognize emulators when we performed attacks on real-time tracking. More powerful emulators might be needed


==> old_framework/cases.tex <==
% USE CASES

==> old_framework/categorization.tex <==
\section{Categorization}
\label{sec:categorization}

This section describes the categorization of apps and attacks according to the data type they target:

\begin{itemize}
    \item \textbf{Safety} 
    \begin{itemize}
        \item Neighbors by ring
    \end{itemize}
    
    \item \textbf{Pricing} 
    \begin{itemize}
        \item Basket Savings
        \item Gas Buddy
    \end{itemize}
    
    \item \textbf{Finding} 
    \begin{itemize}
        \item Where is Public Toilet
        \item Police Detector
    \end{itemize}
    
    \item \textbf{Fitness and Health} 
    \begin{itemize}
        \item Map My Run
        \item Strava
        \item Fitbit
    \end{itemize}
    
    \item \textbf{Family History} 
    \begin{itemize}
        \item My Heritage
        \item Ancestry
    \end{itemize}
    
    \item \textbf{Navigation} 
    \begin{itemize}
        \item Transit
    \end{itemize}
    
\end{itemize}

  

Alternatively, they can also be categorized using the input type needed for attack but the aforementioned categorization is preferred. The input type categorization is as follows:

\begin{itemize}
	
	\item \textbf{Text} 
    
		\begin{itemize}
        \item Neighbors
        \item Basket
        \item Gas Buddy
        \item My Heritage
        \item Ancestry
    \end{itemize}

	\item \textbf{Text and Sensors} 
		  
		\begin{itemize}
        \item Transit
		\end{itemize}

    \item \textbf{Options (text-optional)} 
			
		\begin{itemize}
        \item Where is Public Toilet
        \item Strava
		\end{itemize}

	\item \textbf{Options (text-optional) and Sensors} 
    \begin{itemize}
			\item Map my Run
			\item Strava
      \item Fitbit App
    \end{itemize}

\end{itemize}


==> old_framework/methodology.tex <==
\section{General-Methodology}
\label{sec:methodology}

%----------------------------------------------------------------
\subsection*{Safety}
\begin{itemize}
    \item \textbf{Goal: } \\
    To create terror and confusion in people.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item Fake crime event is created.
        \item Fake event is pushed to the app.
        \item If the fake event is rejected, its modified slightly and pushed again to the app.
        \item If its accepted, move back to step-1 and keep iterating until the desired the number of fake events have been pushed to the app.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\subsection*{Pricing}
\begin{itemize}
    \item \textbf{Goal: } \\
    To create confusion in people and to divert customers either away or towards any particular store or gas-station.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item A list of most popular items on a store or all gas-types for a gas-station is created.
        \item The given store or gas-station is selected in the app.
        \item We iterate through the list of items created earlier and increase or decrease price of each item by 20 percent.
        \item If the desired affect of diverting customers is not achieved, repeat previous step.
        \item If the desired affect of diverting customers is achieved, stop here.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\subsection*{Finding}
\begin{itemize}
    \item \textbf{Goal: } \\
    \\ To confuse people and make them go through secluded areas where the attacker can subject them to further harm like robbery.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item Figure out a busy area thats close to a secluded place.
        \item Re-arrange the objects that the app helps the users in locating in a way that the users go to the secluded place in order to find or avoid the thing shown in app.
        \item Once a user comes to the secluded place, subject them to further harm like robbery or scamming.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\subsection*{Family History}
\begin{itemize}
    \item \textbf{Goal: } \\
    To fool people about their ancestry and act as their fake relatives to further scam them.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item Get access to a persons close ancestry.
        \item Create a fake account on the app and replicate some of their ancestry tree precisely into your relationships.
        \item Contact them and match your ancestry tree with them to fool them into believing you are their unknown relative.
        \item Subject them to elaborate scamming.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\subsection*{Fitness and Health}
\begin{itemize}
    \item \textbf{Goal: } \\
    To win free rewards and prizes at competitions without actually doing the physical activity.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item Take part in competitions and challenges on app that have rewards or prizes of monetary value.
        \item Simulate fake run on the app by spoofing gps location.
        \item Keep repeating previous step until the goal of the competition or challenge has been achieved.
        \item Get the reward or prize without doing actual physical activity.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\subsection*{Navigation}
\begin{itemize}
    \item \textbf{Goal: } \\
    To disrupt real traffic and transit systems by creating fake congestion on roads and fake delays in transit systems.
    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item Create a lot of ghost passengers/riders by creating a lot of emulators.
        \item Spoof gps location on these emulators to a road or train track and keep changing it to simulate movement.
        \item Change it slowly compared to the actual speed of cars or the train to fake the app into believing their is congestion or road or train is delayed.
    \end{enumerate}
\end{itemize}

%----------------------------------------------------------------
\iffalse
\subsection*{}
\begin{itemize}
    \item \textbf{Goal: } \\

    \item \textbf{Steps: } \\
    \begin{enumerate}
        \item 
    \end{enumerate}
\end{itemize}
\fi


==> tables/all_apps.tex <==
\begin{table*}[!ht]
\small
\label{tab:appDetails}
\caption{Crowdsourcing mobile applications}
\begin{tabular}{p{0.025\textwidth} | p{0.1\textwidth} | p{0.5\textwidth} | p{0.1\textwidth} | p{0.1\textwidth}}
  & Title          & Description & Functionality             & Installation Count (Android) \\ \hline
1  & Neighbors by Ring               &             &    Safety                       &  1,000,000+                  \\ \hline
2 & Basket Savings      &             & Money Saving              &                    \\ \hline
3 & Gas Buddy             &             & Money Saving                           &                    \\ \hline
4  & Police Detector               &            &   Location-based utility                         &                    \\ \hline
5  & Where is Public Toilet               &            &   Location-based utility                          &                    \\ \hline
6 & Strava   & Strava is an app tracking your running, cycling or swimming . Your speed, length, time are recorded. You can share your routine with your friends and see the ranking among your friends. You are able to join different kinds of clubs and compete with other people. Your achievements will appear on the leaderboard if you are one of the top 100.
            & Health \& Fitness &      10,000,000+              \\ \hline
7 & Fitbit           & Fitbit is a fitness app recording your all-day activity. For activity, it can record walk, Hike and Run. You can share your achievements with people in different groups
            & Health \& Fitness &      10,000,000+              \\ \hline
8 & Run with Map My Run  &             &  Health \& Fitness            &                    \\ \hline
9  &  MyHeritage             &             &  Family History                         &                    \\ \hline
10  &  Ancestry.com               &             &  Family History                          &                    \\ \hline
11 & Transit        & Transit uses real-time crowding information to estimate commute times for public transportation.\ignore{can update bus/train expected arrival times is a positioning and navigation map in which you can search the real-time routine from the start point to the destination. It also shows the upcoming departure times for all nearby transit lines such as buses and trains. By starting “GO” mode, you will share your routine with other people and see how many people you are influencing.} 
           & Transportation/ Navigation &  5,000,000+          \\ \hline
\ignore{12 & Waze           &    Waze tells you about traffic, roadworks, police, accidents, and more in real-time. If traffic is bad on your route, Waze will change it to save you time.         & Transportation/ Navigation &     100,000,000+               \\ \hline}
\end{tabular}
\end{table*}
